Should You Mask 15% in Masked Language Modeling?

Masked language models (MLMs) conventionally mask 15% of tokens due to the belief that more masking would leave insufficient context to learn good representations; this masking rate has been widely used, regardless of model sizes or masking strategies. In this work, we revisit this important choice of MLM pre-training. We first establish that 15% is not universally optimal, and larger models should adopt a higher masking rate. Specifically, we find that masking 40% outperforms 15% for BERT-large size models on GLUE and SQuAD. Interestingly, an extremely high masking rate of 80% can still preserve 95% fine-tuning performance and most of the accuracy in linguistic probing, challenging the conventional wisdom about the role of the masking rate. We then examine the interplay between masking rates and masking strategies and find that uniform masking requires a higher masking rate compared to sophisticated masking strategies such as span or PMI masking. Finally, we argue that increasing the masking rate has two distinct effects: it leads to more corruption, which makes the prediction task more difficult; it also enables more predictions, which benefits optimization. Using this framework, we revisit BERT's 80-10-10 corruption strategy. Together, our results contribute to a better understanding of MLM pre-training.

==> sections/mask_more.tex <==
%!TEX root = ../main.tex



% \input{tables/maintable.tex}
% \input{tables/maintabledev.tex}


% \input{tables/maskrate_example.tex}

%
% \danqi{Now I think the main result table (Table 4?) should be moved here now..}
% \tianyu{I think the best way is either (1) we put a large table here but ony with our 15\%/40\%, or (2) we leave the table in the end but we can have comparison with bert-base/large/academic bert with both test nubmers and time. Putting a table with a lot of weirdly connected baseline here will make the message unclear.}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.99\textwidth]{figures/15_vs_50_reptask.pdf}
%     \caption{Downstream task performance of \ttt{large} models trained with academic BERT recipe, under masking rates of 15\% and 50\%. We report accuracy for MNLI, QNLI, QQP, SST-2, Spearman's correlation for STS-B, and F1 for SQuAD. 50\% outperforms 15\% or achieves comparable performance for the majority of the tasks.}
%     \label{fig:15_vs_40_reptask}
% \end{figure*}



% We first train two \ttt{large} models from scratch using the academic BERT recipe, with a masking rate of 15\% and 50\% respectively. We then evaluate the models on downstream tasks and plot the downstream performance with respect to steps in Figure~\ref{fig:15_vs_40_reptask}.

% \danqi{I am not quite sure why we need such a big figure with $x$-axis = \# of training steps. Do we want to make a point that 50\% masking rate has a bigger advantage at earlier steps? Unclear from the figure.}

% Surprisingly, although masking half of the context, the 50\% masking rate model still outperforms the 15\% model, or achieves on par performance, on most tasks.
% This observation suggests that the canonical 15\% masking rate may be suboptimal, and the model can still learn meaningful -- or even better -- representation given a highly corrupted context.
% Figure~\ref{fig:large_mask} shows the performance change with respect to different masking rates.

% We then further study under different model sizes, different training steps, and different masking policies\danqi{what are policies?}, what the optimal masking rate should be.
% The following results not only offer an empirical guideline for masking rates,
% but also shed some light on the inner workings of masked language modeling.


% (complete results are in Appendix~\ref{sec:app:more_mask_rate}).
%\alex{This is weird given Figure~\ref{fig:large_mask} doesn't use ``train-longer''}).
%\zexuan{Figure 1 only shows results with masking rates from 15\% to 50\%. It looks like we don't include results with larger rates like 90\%?}
% Table~\ref{tab:maskrate_example} shows several masking rates and examples of masked sentences, along with the training perplexity and downstream performance.

 % (complete results are in Appendix~\ref{sec:app:more_mask_rate}).
%\alex{This is weird given Figure~\ref{fig:large_mask} doesn't use ``train-longer''}).
%\zexuan{Figure 1 only shows results with masking rates from 15\% to 50\%. It looks like we don't include results with larger rates like 90\%?}
% Table~\ref{tab:maskrate_example} shows several masking rates and examples of masked sentences, along with the training perplexity and downstream performance.


==> sections/old_analysis.tex <==
%!TEX root = ../main.tex

\section{Analysis}
\label{sec:analysis}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figures/mlm_15_vs_50.pdf}
    \caption{MLM 15\% vs 50\%. {\color{green}Green} represents correct prediction; {\color{orange}orange} represents different prediction from ground-truth but making sense; {\color{red}red} represents completely wrong predictions.\tianyu{draft for now.} \alex{I still think the $\langle / s \rangle$ is weird.}}
    \label{fig:mlm_15_vs_50}
\end{figure*}

How does a model benefit from masking rates of up to $50\%$?
How can it learn useful features, given its predictions are often ungrammatical guesses, as independent predictions cannot capture the complex inter-correlated distribution of all the masked tokens? \alex{(see Figure?)}
We tackle these questions with carefully designed ablation experiments.

\input{tables/corruption_pred.tex}

\subsection{Disentangling Masking into Corruption and Prediction}
\label{sec:corruption_and_prediction}

The masking rate $m$ determines two import aspects of the pre-training problem. Given a token sequence of length $L$:
(1) In the data pre-processing, we corrupt $\lfloor m_{corrupt} L \rfloor$ of the input tokens, such that the mutual information between the masked inputs and their targets is zero. Typically, this is done by substituting [MASK].
\tianyu{Maybe avoid jargons like mutual information?} \alex{fair}
(2) The model makes $\lfloor m_{predict} L \rfloor$ predictions about the original identity of the masked tokens. During training, a cross-entropy loss is computed at each position.

Usually, masking and prediction rates are coupled, such that $m_{corrupt} = m_{predict}$, but they may impact representation quality differently.

\paragraph{\boldmath{$m_{corrupt}$} controls task difficulty.}
Masked language modeling attempts to learn a conditional probability distribution over the vocabulary $p(masked\;token | context)$ during pre-training.
If a larger proportion of the input is corrupted, a token prediction is conditioned on less context tokens, making predictions harder and more uncertain.
We argue that this is why larger models with more capacity are better at learning with larger masking rates.

\paragraph{\boldmath{$m_{predict}$} relates to optimization.}
Each prediction leads to a loss gradient, which is averaged to optimize the weights of the model.
Averaging across more predictions reduces stochastic gradient noise, giving a more accurate estimate of the gradient.
\citep{liu2019roberta} found that language models benefit from large batch sizes, which gives more predictions per gradient step.
A higher prediction rate is another way to increase the predictions per step.
Additional predictions share the same context, and will not be as informative as additional sequences in a batch.
However, as opposed to increasing the batch size, they can be obtained at almost no extra cost.

\paragraph{Experiments}
When tuning the masking rate in our experiments, we set $m = m_{corrupt} = m_{predict}$.
Here, we propose a method that allows $m_{corrupt}$ and $m_{predict}$ to vary independently.
This disentangles the effects of $m_{corrupt}$ and $m_{predict}$ on our results.

There are two distinct cases:
\begin{enumerate}
    \item If $m_{predict} < m_{corrupt}$, the loss is computed on only a subset of the masked tokens.
    \item If $m_{predict} > m_{corrupt}$, we duplicate a sequence $\lceil \frac{m_{predict}}{m_{corrupt}} \rceil$ times and sample disjoint sets of $\lfloor m_{corrupt}L \rfloor$ masks in the different sequences. This allows additional predictions at a lower corruption rate while keeping the training input constant.\footnote{This ablation is also $\lceil \frac{m_{predict}}{m_{corrupt}} \rceil$ times as computationally expensive as the baseline setting $m_{predict} = m_{corrupt}$.}
\end{enumerate}

Keeping either $m_{corrupt}$ or $m_{original}$ at 40\%, we find that our model primarily benefits from better optimization, while lower $m_{corrupt}$ rates are beneficial given equal optimization.
Note that this ignores training time, as lower $m_{corrupt}$ at high $m_{predict}$ is much slower given equal computational resources.

% \tianyu{Better understand what the masking rates are: disentangle it into corruption and prediction. We show that higher prediction rates lead to better performance, while corruption rates are correlated to task difficulty.
% It corresponds to the previous two findings that we made.
% }

\paragraph{Same Token Predictions}
\citet{devlin2019bert} suggests that it is beneficial to substitute the original token for 10\% of cases instead of [MASK].
% [MASK] for only 80\% of masked tokens, leaving a random token or the original token in 10\% of cases respectively.
This is intended to reduce the discrepancy to the downstream task and almost all subsequent works follow this guideline.
% \alex{As our masking strategy drastically increases this discrepancy, we re-evaluate the effectiveness of such mitigation.}

We argue that predicting the same token should neither count towards the corruption nor to the prediction rate. The associated loss decreases rapidly to near zero, which leads to very small gradients and contributes little to optimization. We should rather think of this objective as an auxiliary regularization loss, which ensures that some token information is propagated from the embeddings to the final layer.
In this framework, BERT actually uses a masking rate of 13.5\%.

Empirically, we find that regularization from additional same token predictions consistently helps for some tasks, while deteriorating performance on others. \danqi{Sorry, this point is good but I don't see which results support it. } Our results are summarized in Table \ref{tab:same_ran}.
We hypothesize that there is a trade-off between exposing contextualized features and per-token features, that is controlled via the same token prediction rate.
Replacing existing [MASK] tokens with the original tokens hurts performances more, which in our framework lowers the masking rate, consistent with our main finding that larger masking rates are beneficial.

\danqi{This paragraph is too long}

\paragraph{Random Token Corruptions}
Additionally, \citet{devlin2019bert} replace [MASK] with the original\danqi{original or random} token in 10\% of cases.
% [MASK] for only 80\% of masked tokens, leaving a random token or the original token in 10\% of cases respectively.
Random mask tokens contribute to corruption and prediction rate, as there is no information leakage between input and output. In fact, loss is slightly higher on random tokens compared to [MASK]s, as predictions need to be invariant to large variations in the input.
\alex{could mention connection to ELECTRA, as it leads to the auxiliary task of replaced token identification.}

In our ablation experiments in Table \ref{tab:same_ran}, we find that replacing [MASK] tokens with randomly sampled tokens consistently deteriorates performance (in terms of perplexity and downstream accuracy).

% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=0.98\textwidth]{figures/pred_vs_mask.pdf}
%     \caption{Pred vs. mask. \alex{Maybe turn this into a table? I don't think intermediate checkpoints are interesting. And add pred20+mask20 and pred40+mask10.}}
%     \label{fig:pred_vs_mask}
% \end{figure*}

\label{sec:same_random}


\input{tables/same_ran.tex}

\paragraph{Discrepancy To Downstream Task}
More corruption leads to greater distributional shift from pre-training to downstream.
We find that transformer architecture can quickly adapt to full, uncorrupted sentences, regardless of the masking rate.
- Show linear probing results
- Show few-shot results
Table~\ref{tab:few_full}

\input{tables/few_full.tex}

\paragraph{More Corruption Prevents Shortcuts}
% \label{sec:pmi}
\citet{levine2021pmimasking} conjecture that many masked predictions can be made sorely based on local ``shortcut'' cues, such as intra-word and inter-word collocations.
As a remedy, they propose a masking strategy which masks spans of correlated words as one unit, requiring extensive pre-processing.
We estimate the expected number of such spans which get masked entirely with a uniform masking strategy, and find that the odds
increase X-fold when raising the masking rate from 15\% to 40\%.
Similarly, we mask a much greater number of completely masked words.
It is an example of how the increased task difficulty may induce better representations.
\alex{note that span masking increases task difficulty and optimal masking rate}

\todo{Add figure...}


\subsection{Processing to ``see'' the masks}

\begin{itemize}
    \item Show the performance of baseline vs. disabling attention (large 24h recipe 40\%) (Table).
\end{itemize}

% \tianyu{Combine to the next subsection?}

\tianyu{Show that it is crucial to have the attention from the masked tokens to the unmasked tokens.}

\alex{Difference to vision: masks may learn skills, not only representations}

\tianyu{add the 90\% 100\% masking results, random initialized baseline, unigram baseline}

\tianyu{For 100\% masking, test the probability of turn on and turn turn.}

% \subsection{Independent decoding is fine}
% \alex{Why 50$\%$ works and how it compares to T5}
% \alex{I'm really not sure what to write here}
% Lower bound to loss:
% \begin{align*}
%     &D_{KL}\left(p(\cup_{i \in M} y_i | context) \middle\| \prod_{i \in M} p(y_i | context)\right) \\
% = &I(Y_1; ...; Y_{M} | context)
% \end{align*}
%
% \tianyu{Let's remove this section and move any discussion related to T5 to related work/discussion.}

% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=0.98\textwidth]{figures/attn_disabled.pdf}
%     \caption{Disable attention from masks to unmasked tokens.}
%     \label{fig:disable_attention}
% \end{figure*}
%
%


==> sections/old_mask_rate_dep_.tex <==
%!TEX root = ../main.tex

% \section{Masking Rate Comparison}
\section{Masking 50\% Can Be Better than 15\%}

\label{sec:mask_rate}

\tianyu{This section is to show the main finding 1: we can train models more efficiently with higher masking rates.}

% \tianyu{Show the results of different mask rates. Figures of selected tasks: MNLI, QNLI, QQP, STS-B, SST-2, SQuAD. Full tables in the appendix. }

\subsection{Academic BERT recipe}

\tianyu{We show that with the large model and the academic bert recipe, 50\% is better than 15\% and 40\% is the optimal.}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/large_mask_to_perf.pdf}
    \caption{Large mask rate.}
    \label{fig:mask_rate_large}
\end{figure*}

\begin{itemize}
    \item Show the performance - masking rate figure with the 24h large model (Figure~\ref{fig:mask_rate_large}).
    \item Show the performance - step figure with 15\%, 40\% and 50\% masking rates with the 24h large model. 
\end{itemize}

\subsection{Train longer}

\tianyu{We show that when training longer (either 24h recipe or original recipe), 15\% and 40\% perform similarly.}

\begin{itemize}
    \item Show the performance - step figure of the large model original recipe results, with 15\% and 40\% masking rates.
    \item Show the performance - step figure of the large model 24h recipe results (train longer), with 15\% and 40\% masking rates.
\end{itemize}

\tianyu{Do we want to add the masking rate scheduling?}

% Large model with different mask rates: Table~\ref{tab:mask_rate_large}
% 
% Base model with different mask rates: Table~\ref{tab:mask_rate_base}
% 
% Large model figure: Figure~\ref{fig:mask_rate_large}

% \input{tables/mask_rate_large.tex}
% \input{tables/mask_rate_base.tex}


% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=0.98\textwidth]{figures/base_mask_to_perf.pdf}
%     \caption{Base mask rate.}
%     \label{fig:mask_rate_base}
% \end{figure*}


==> sections/old_observation.tex <==
%!TEX root = ../main.tex

\section{Mask More Than 15\%}
\label{sec:observation}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figures/15_vs_50_reptask.pdf}
    \caption{Downstream task performance of \ttt{large} models trained with academic BERT recipe, under masking rates of 15\% and 50\%. We report accuracy for MNLI, QNLI, QQP, SST-2, Spearman's correlation for STS-B, and F1 for SQuAD. 50\% outperforms 15\% or achieves comparable performance for the majority of the tasks.}
    \label{fig:15_vs_40_reptask}
\end{figure*}
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.99\textwidth]{figures/large_mask.pdf}
    \caption{Impact of masking rates to \ttt{large} models with academic BERT recipe. \danqi{Definitely need to put 15\% in the $x$-axis. I feel we can even draw a horizontal line there showing 15\% as the baseline. Add multiple runs for SQuAD.}}
    \label{fig:large_mask}
\end{figure*}

We first train two \ttt{large} models from scratch using the academic BERT recipe, with a masking rate of 15\% and 50\% respectively. We then evaluate the models on downstream tasks and plot the downstream performance with respect to steps in Figure~\ref{fig:15_vs_40_reptask}.  \danqi{I am not quite sure why we need such a big figure with $x$-axis = \# of training steps. Do we want to make a point that 50\% masking rate has a bigger advantage at earlier steps? Unclear from the figure.}

\danqi{I don't see Figure 2 is quite useful. I wonder if we should just present results with 50\%-90\% in one table? Another option is to combine it with Figure 3?}

Surprisingly, although masking half of the context, the 50\% masking rate model still outperforms the 15\% model, or achieves on par performance, on most tasks.
This observation suggests that the canonical 15\% masking rate may be suboptimal, and the model can still learn meaningful -- or even better -- representation given a highly corrupted context.
Figure~\ref{fig:large_mask} shows the performance change with respect to different masking rates.

We then further study under different model sizes, different training steps, and different masking policies\danqi{what are policies?}, what the optimal masking rate should be.
The following results not only offer an empirical guideline for masking rates,
but also shed some light on the inner workings of masked language modeling.

\subsection{Model sizes and masking rates}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/model_size_mask_normalize_qqp.pdf}
    \caption{Impact of masking rates on difference model sizes. We see that larger models favor larger optimal masking rates.
    %\alex{order oat milk + get rid off std. dev. for averaged results OR compute the std. dev. for the average, assuming that the noise in different tasks is independent, and plot that.}
    \danqi{Can change QQP to SQuAD? Just make it consistent with other figures. Also the variances seems to be large on QQP.}
    }
    \label{fig:model_size_mask_normalize_qqp}
\end{figure}

We find that \textbf{larger models possess higher optimal masking rates.} \danqi{I will use the bold text as section titles directly. Important messages!}
Figure~\ref{fig:model_size_mask_normalize_qqp} demonstrates the impact of masking rates on \ttt{large}, \ttt{base}, and \ttt{medium} models.\danqi{Need to specify model sizes somewhere -- I still find it not intuitive that medium is smaller than base. Any tweaks here?}\footnote{For each task and each model size, \emph{normalized performance} is calculated by $\frac{x-x_{15\%}}{\sigma}$ where $x_{15\%}$ is the performance of 15\% masking rate and $\sigma$ is the standard deviation across all masking rates.
}
We see that under the academic BERT recipe, on average, \ttt{large} models take 40\% as the optimal masking rate; \ttt{base} models take 30\% as the optimal masking rate; \ttt{medium} models take 20\% as the optimal masking rate.
This clearly shows that models with larger capacity benefits more from higher masking rates.

% To understand the reason behind it, in \S\todo{} we disentangle the masking rate as corruption rate and prediction rate. While all models benefit from more predictions, we show that models with larger capacity can handle higher corruption rates\todo{we have no experiments for that}, and thus favor higher masking rates.
% \alex{link to efficiency and train large: then compress}

\tianyu{Discuss the relation to efficient pre-training, here or in discussion section.}
We also link our findings to those of \citet{li2020train,izsak2021train} -- large models converge significantly faster, and training large models and stopping early is a more efficient strategy.
By using our findings of adopting higher masking rates with large models -- which leads to better performance at the early stage of pre-training -- we make the large model recipe even more efficient. \danqi{I don't see how you made this point of ``at the early stage''.}



\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/mask_strategy_mask_normalize_squad.pdf}
    \caption{Different masking strategies trained with different masking rates (academic BERT recipe, \ttt{large} models). \todo{Add wholeword and pmi (squad is still running).}} \alex{weird PMI and whole word performance on squad for 15\%}
    \label{fig:mask_strategy_mask_normalize_qqp}
\end{figure}


\subsection{Masking strategies and masking rates}

We show that \textbf{
uniform sampling with higher masking rates performs better than or on par with more sophisticated masking strategy.
}
\alex{what to highlight: (1) comparing masking strategies at 15\% is misleading, uniform masking at 40\% can be much stronger. (2) even when tuning masking rate for other masking schemes, uniform masking is competitive. (3) interesting: other masking schemes have lower optimal masking rate}
The vanilla MLM pre-training uniformly samples the position of mask tokens.
Recently, a series of new masking strategies emerge to improve the performance of MLM,
namely whole word masking~\cite{devlin2019bert}, span masking~\cite{joshi2020spanbert,raffel2020exploring}, and PMI masking~\cite{levine2021pmimasking}.
The idea of those strategies is to mask consecutive words with a higher probability to avoid trivial masks and they are shown to outperform uniform sampling on downstream tasks.

We study how the optimal masking rates and the downstream performance change given different masking strategies (Figure~\ref{fig:mask_strategy_mask_normalize_qqp}).
We find that
(1) the optimal masking rates for whole word/span/pmi masking are lower than the uniform one;
(2) even though the advanced masking strategies have advantage at 15\% masking, the uniform masking achieves comparable or even better results when at its optimal masking rate.

\alex{Maybe we should rather have plots over training steps rather than masking rate; and show that uniform at 40\% is superior to span/PMI masking at 15\% and 40\%.}

To understand the relation between higher masking rates and advanced masking strategies,
we show in \S\todo{} that more uniform masking essentially increases the chance of masking highly-correlated tokens,
which reduces trivial mask tokens and potentially forces the model to learn more robustly.

% To understand why higher masking rate makes uniform masking better than other advanced masking strategies,
% we analyze how masking rates change the average continuous span lengths of the masked tokens in Figure \todo{}.


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figures/train_long_15_vs_40.pdf}
    \caption{15\% vs 40\% masking rates with \ttt{large} models, academic BERT recipe but trained longer. \danqi{Forgot -- What is the reason that we don't have multiple runs for SQuAD?} \tianyu{It's because SQuAD is quite stable and conventionally people don't use mutliple seeds. But we are now running on multiple seeds just to make figures better/consistent.} \tianyu{SQuAD still running.}}
    \label{fig:train_long_15_vs_40}
\end{figure*}






\subsection{Training steps and masking rates}

\danqi{I kinda want to suggest to downweigh this section and leave it in appendix to back up that our conclusions don't just  depend on AcademicBERT.}

We find that
\textbf{
fewer training steps prefers higher masking rates.
}
To study the relation between training steps, masking rates, and downstream performance, we train the \ttt{large} models with academic BERT recipe, but with longer training steps.\footnote{
See Appendix \todo{} for a comparison between out recipe and the original BERT/RoBERTa recipe.
}
Figure~\ref{fig:train_long_15_vs_40} shows the performance change with respect to different training steps of both 15\% and 40\% masked models.
For the majority of the tasks, the 40\% model has larger advantage over the 15\% model at the 25k step, compared to the 125k step.
This shows that with longer training time, the efficiency boost by masking/predicting more fades.
Even though, we see on QNLI, STS-B, and SST-2, the higher masking model performs better with 125k step training.

\danqi{Hmm, Figure 2 and Figure 6 look very similar... It is quite surprising that the trend of SST-2 is flipped in both figures. I don't know what conclusion you want to draw here --- The orange curve is still above blue curve in most datasets, right? Why is MNLI an exception?}


==> tables/few_full.tex <==
%!TEX root = ../main.tex

\begin{table}[h]
    \centering
    \resizebox{0.98\linewidth}{!}{
        \begin{tabular}{lcccc}
            \toprule
            & MNLI &  QNLI & QQP & SST-2  \\
            \midrule
            \multicolumn{5}{c}{1,000-shot} \\
            \midrule
            15\% & \tf{60.40 (0.08)}	&	\tf{80.20 (0.64)}&	\tf{77.13 (0.46)}&	\tf{87.40 (0.42)} \\
            40\% & 59.77 (0.96)	&	\tf{80.73 (1.14)}&	74.57 (1.64)&	86.27 (0.78)\\
            \midrule
            \multicolumn{5}{c}{Full dataset}\\
            \midrule
            15\% & 84.20 (0.08)	&	90.87 (0.26) &	87.77 (0.05) &	\tf{93.30 (0.28)}\\
            40\% & \tf{84.50 (0.08)}	&	\tf{91.55 (0.11)} &	\tf{88.10 (0.00)} &	92.83 (0.12) \\ 
            \bottomrule
        \end{tabular}
    }
    \caption{Few-shot vs full.}
    \label{tab:few_full} 
\end{table}

==> tables/mask_rate_base.tex <==
%!TEX root = ../main.tex

\begin{table*}[!t]
    \centering
    \resizebox{0.98\textwidth}{!}{
        \begin{tabular}{lcccccccccccc}
            \toprule
            & MNLI & M-mm & QNLI & RTE & QQP & MRPC & STS-B & SST-2 & MR & CoLA & SQuAD \\
            \midrule
            15\% & 81.90&	82.33&	88.80&	57.77&	86.73&	71.70&	86.09&	91.47&	85.73&	51.17&\\
            20\% & 81.90&	82.50&	89.24&	65.67&	87.13&	72.70&	86.20&	91.70&	85.67&	50.00&\\
            30\% & 82.10&	82.40&	89.53&	60.77&	87.20&	68.73&	85.68&	92.20&	85.90&	49.57&\\
            40\% & 82.15&	82.27&	89.53&	58.37&	87.00&	69.07&	84.24&	92.27&	84.97&	48.50&\\
            50\% & 81.70&	82.27&	89.30&	58.40&	87.07&	68.93&	85.03&	91.30&	84.53&	49.60&\\
            \bottomrule
        \end{tabular}
    }
    \caption{Different masking rate with the \ttt{base} model.}
    \label{tab:mask_rate_base}
\end{table*}


==> tables/mask_rate_large.tex <==
%!TEX root = ../acl.tex

\begin{table*}[ht]
    \centering
    \resizebox{0.98\textwidth}{!}{
        \begin{tabular}{lcccccccccccc}
            \toprule
            & MNLI & M-mm & QNLI & RTE & QQP & MRPC & STS-B & SST-2 & MR & CoLA & SQuAD \\
            \midrule
            15\% & 84.20&	84.63&	90.87&	67.27&	87.77&	76.97&	87.67&	93.30&	87.60&	59.17&	83.31	\\
            20\% & 84.13&	84.63&	91.27&	66.90&	87.93&	78.83&	87.38&	92.67&	87.17&	60.13&	84.16&	\\
            30\% & 84.23&	84.77&	91.63&	68.33&	87.97&	76.13&	88.47&	93.03&	86.70&	60.60&	84.23&\\
            40\% & 84.50&	84.83&	91.55&	67.00&	88.10&	76.93&	88.24&	92.83&	87.13&	61.00&	84.92&\\
            50\% & 84.07&	84.27&	91.13&	68.10&	88.07&	76.73&	87.63&	92.73&	87.00&	57.87&	84.19&\\
            60\% & 83.20&	83.90&	90.70&	68.23&	87.80&	76.27&	87.62&	92.57&	86.13&	54.47&	83.65&\\
            \bottomrule
        \end{tabular}
    }
    \caption{Different masking rate with the \ttt{large} model.}
    \label{tab:mask_rate_large}
\end{table*}
